ASIACO: Asiago Spectroscopy and Imaging Atlas of COmets

The ASIACO project is an atlas of cometary imaging and spectroscopy obtained from the Asiago Astrophysical Observatory between 2012 and 2024, still ongoing. Up to now, we monitored 41 comets, acquiring broad-band images using the INAF-OAPd 1.82m Copernico and the 0.67/0.92m Schmidt telescopes, as well as low-to-medium resolution spectra with the DFA-UniPd 1.22m Galileo Telescope. Our dataset offers significant scientific potential, enabling studies on the true extent of cometary tails, orientation of nuclei spin axes, retrieval of compositional data, and determination of production rates for key molecular and atomic species. The Atlas will become publicly available for scientific research, and the project remains active, continuously adding monitored comets.

==> Intro.tex <==
%\section*{Prefaction}
Comets have been studied with the Galileo telescope since 1942, following a long Italian tradition that began with Giovan Battista Donati at Arcetri in the second half of the 19th century. This tradition continued with Antonio Maria Antoniazzi at the Specola of Padua in the early 20th century, and later with Antonino Gennaro, Salvatore Taffara, and Giuseppe Mannino at the Asiago Astrophysical Observatory in the 1950s and 1960s.\\
The Galileo telescope, located at the Asiago Astrophysical Observatory on the Asiago plateau, has a diameter of 1.22 meters ($f/10$) and has made significant contributions to the spectroscopic study of comets. Among the numerous publications on this topic, one worth mentioning is the work of Piero Benvenuti and Karl Wurm (1974), which describes the discovery of a pair of "doublets" in the spectra of the comet Kohoutek (C/1973E), later identified by G. Herzberg and H. Lew (1974) as originating from the H$_2$O$^+$ ion. Also noteworthy is a publication of a few years earlier by G. Mannino, concerning the spectroscopic analysis of the comet Mrkos (1957D), where he announced the rare detection of an intense emission "doublet" due to sodium (Na). \\
In the last 10 years, equipped with a Boller \& Chivens spectrograph, the Galileo telescope has been effectively used to monitor dozens of comets (with a magnitude $< 16$), making use of all the available gratings.

\begin{table}[h!]
    \centering
    \begin{tabular}{|c c c c c|}
        \hline
        \textbf{Lines/mm} & \textbf{Blaze wavelength} & \textbf{Dispersion} & \textbf{Spectral Range} & \textbf{Observable Emissions}\\
         & [\AA] & [\AA/px] & [\AA] & \\
        \hline
        \hline
        300 & 5000 & 2.25 & 4600 & CN, C$_2$ (Swan bands), NH$_2$ bands \\
        600 & 4500 & 1.15 & 2300 & C$_2$ (Swan bands), NH$_2$ bands, O I\\
        1200R & 4000 & 0.6 & 1200 & CN, C$_2$ (Swan bands)\\
        1200B & 6825 & 0.6 & 1200 & Na I, O I, NH$_2$, H$_2$O$^+$, H$\alpha$\\
        \hline   
    \end{tabular}
    \caption{}
    \label{tab:gratings}
\end{table}

\noindent The back-illuminated ANDOR iDus DU440A E2V 42-10 sensor and the altitude of the Asiago Astrophysical Observatory (1045 meters above sea level) allow for spectral readings from almost 3300 Å to beyond 7500 Å, where fringing, a typical problem of a thin sensor, comes into play.\\
\noindent With the desire to celebrate the 80th anniversary of this grand telescope's service (inaugurated in 1942), we present a summary of the spectroscopic observations of comets over the last decade, accompanied by images obtained almost simultaneously with the other INAF-OAPd telescopes at the Asiago Astronomical Station (the 182 cm Copernico telescope and the 67/92 cm Schmidt telescope). \\

\noindent The idea for the creation of this volume was born from the Authors' desire to make available to the entire scientific community the numerous cometary spectra obtained with the high quality of the Galileo telescope. The pages of this volume are enriched with images taken mainly with in the $BVri$ photometric filters (reduced and calibrated); everything is in paper format but also made digitally accessible to interested parties on the dedicated website created in support to the volume.\\
The work for the creation of this database, made possible thanks to the direct contribution of several students of the Master Degree in Astronomy from the Universities of Padua and Trento, also carries significant educational value for these students. Our publication is linked to three objectives:
\begin{itemize}
    \item Relaunch the spectroscopic study of comets with the Galileo telescope.
    \item Facilitate the use of the extensive archive of science data that has been accumulated over time.
    \item Continuously increase and expand the database available to the scientific community.
\end{itemize}
This last objective is closely connected to the first and requires the constant use of the Galileo telescope, as well as the establishment of a `human' task force to address the needs of the database.\\
Research activities in the field of comets can and should be a flagship endeavor! Over time, it has also become a fundamental tool for educational and scientific outreach activities for the general public, who increasingly attend the Asiago Astronomical Observatory. This includes the discovery of the allure `radiated' by comets, which are quite common visitors of the inner Solar System, but for many people, they remain mysterious and fascinating objects.
\newpage
\section{THE GALILEO TELESCOPE AND ITS INSTRUMENTATION}
The 122-cm telescope at the Asiago Astrophysical Observatory was built by the Galileo Officine in Florence between 1940 and 1942 and dedicated to Galileo Galilei on the occasion of the third centenary of his death. At that time, it was the largest telescope in Europe. It was originally designed with two optical configurations: Newton and Cassegrain. However, the telescope is now only used in the Cassegrain configuration with a hyperbolic secondary mirror with a diameter of 52 cm.
The aluminization of the Galileo telescope's mirrors is periodically carried out in a vacuum chamber located in the nearby workshop of the Cima Ekar Astronomical Observatory (Asiago).
Since 1998, a Boller \& Chivens spectrograph has been permanently mounted at the Cassegrain focus. It was manufactured by Perkin Elmer (model 58770). The B\&C spectrograph features a slit at the Cassegrain focal plane with a variable aperture of up to 1 mm and a length of 28 mm.
The collimator for directing the optical beam onto the grating is an off-axis parabolic mirror with a diameter of 90 mm and a focal length of 810 mm. A set of 4 gratings with dispersions ranging from 42 Å/mm to 339 Å/mm completes the equipment of the spectrograph.
The dispersed light beam is directed toward the Dioptric Blue Galileo Camera with a focal length of 188 mm, and it operates in conjunction with an Andor iDus DU440 CCD camera with a 2048×512 pixels sensor. The spatial resolution on the CCD is 1"/pixel. Several comparison lamps are permanently installed to enable wavelength calibration of the spectra.
The side of the slit facing the incoming light beam has a reflective surface. On this surface, the image produced by the telescope is reflected to be captured by the guide camera (Andor iXon DV885 with an EMCCD sensor); the field of view is 8.5' × 6.4' with a resolution of 0.68"/pixel.
The telescope tracking movement has been implemented with differential tracking, allowing it to autonomously track the motion of celestial objects (comets, in our case) that do not move at sidereal speed.

\subsection{GALILEO TELESCOPE TECHNICAL DATA}
Values related to the intersection between the polar axis and the declination axis of the telescope:
\begin{table}[h!]
    \centering
    \begin{tabular}{|l c|}
        \hline
        Longitude: &  E 11$^{\circ}$31$^{'}$35.138$^{"}$ \\
        Latitude: & +45$^{\circ}$51$^{'}$59.340$^{"}$ \\
        Altitude: & 1044.2 meters above sea level \\
        International code IAU-MPC: & 043 \\ 
        Primary Mirror Diameter (outer edge): & 1237 mm \\
        Primary Mirror Effective Diameter:    &    1200 mm \\
        Primary Mirror Thickness (at the edge): &  208 mm \\ 
        Primary Mirror Weight:              &      575 kg \\
        Primary Mirror Focal Length:       &       6000 mm \\ 
        Primary Mirror Focal Ratio:        &       $f/$5.0 \\
        Secondary Mirror Diameter:         &       520 mm \\
        Equivalent Focal Length:          &        12100 mm \\
        Focal Ratio:                     &         $f/$10.1 \\
        Scale:                         &           17.05 arcsec/mm \\
       \hline   
    \end{tabular}
    \caption{}
    \label{tab:telescope info}
\end{table}


\newpage
\section{OUR TECHNIQUES}
\subsection{Spectra}
Observational nights have been scheduled in an identical manner: by capturing at least one spectrum of a spectrophotometric standard star from the ESO catalogue \footnote{https://www.eso.org/sci/observing/tools/standards/spectra/stanlis.html},
by capturing a spectrum of a star defined as a "solar analog."
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.25]{img_intro/C2022E3.jpg}
    \caption{Fig.1 Typical spectrum of a comet (C/2022 E3 - monochromatic image from the Galileo telescope). The radiation from the night sky enters across the entire width of the slit and forms vertical lines throughout its height. The wide field framed by the same slit allows for the extraction of the night sky background far away from the emissions of the core region without being contaminated by the brightness of the outer coma.}
    \label{spec_ex}
\end{figure}
The length of the slit (8.5 arcminutes on the celestial plane) has always allowed us to extract the lines of the night sky without "contaminating" the spectrum with the brightness of the comet's coma under examination.
The back-illuminated ANDOR sensor provides excellent performance in the ultraviolet, while suffering from fringing (photons interference) in the near-infrared due to sensor thinning; whenever possible, efforts were made to mitigate this effect by taking and averaging different spectra at different points along the slit.
The IRAF v2.6 software was used for the reduction of all spectra, with the standard calibration for dark, bias signal, and flat field. Wavelength calibration was performed using He-Fe-Ar lamps.
For proper flux calibration, Bolin and Lindler's (1992) ESO Standard Stars were used.
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.2]{img_intro/apall1.jpg}
    \caption{Fig.2 To extract a cometary spectrum, it is necessary to subtract the contribution of the night sky from the raw spectrum. The two side segments adjacent to the peak, indicated in red, represent the areas from which the sky background, far from the contributions of the comet's nucleus and coma, has been "extracted."}
    \label{fig:apall1}
\end{figure}
Only subsequently, the already calibrated spectra were divided by a spectrum of a star known as a "solar analog" (spectral classification G2V), also calibrated in the same manner as the comet spectrum (see Table \ref{tab:SolAn}).
The results published in this volume, therefore, correspond to a relative flux emitted by each comet. This representation method was chosen because the "analysis" allows for a direct and immediate comparison between the spectra of all comets studied at Asiago: briefly, one can identify salient and/or repetitive features in the spectra of the same comet or how these features appear in different comets.

%\begin{figure}[h!]
%    \centering
%    \includegraphics[scale=0.4]{img_intro/slit_img.jpg}
%    \caption{Fig.3 Negative image of the field of view of the guiding camera of the Galileo telescope during a working session on comet C/2020 V2. The white trace corresponds to the position and direction of the spectrograph slit, here set with a width of 200 microns.}
%    \label{fig:slit_img}
%\end{figure}

\begin{table}[h!]
    \centering
    \begin{tabular}{|c c c c|}
        \hline
         \textbf{name} & \textbf{RA} & \textbf{Dec} & \textbf{V mag} \\ 
          & [hh mm ss] & [$^{\circ}$ ' "] & \\
         \hline 
         \hline
         Land(SA) 93-101 & 01 53 18.0 & +00 22 25 & 9.7 \\ 
         Hyades 64 & 04 26 40.1 & +16 44 49 & 8.1\\
         Land (SA) 98-978 & 06 51 34.0 & -00 11 33 & 10.5 \\
         Land (SA) 102-1081 & 10 57 04.4 & -00 13 12 & 9.9 \\
         Landolt (SA) 107-684 & 15 37 18.1 & -00 09 50 & 8.4 \\
         Land (SA) 107-998 & 15 38 16.4 & +00 15 23 & 10.4 \\
         16 Cyg B & 19 41 52.0 & +50 31 03 & 6.2 \\
         Land (SA) 112-1333 & 20 43 11.8 & +00 26 15 & 10.0 \\
         Land (SA) 115-271 & 23 42 41.8 & +00 45 14 & 9.7 \\
         \hline
         
    \end{tabular}
    \caption{Stars defined as solar analogs were used as the divisor in the reduction to "relative flux" of all the spectra taken at the Galileo telescope in Asiago. The figures in the volume depict spectra resulting from the division: (comet flux / Solar Analog flux).}
    \label{tab:SolAn}
\end{table}
%Stars defined as solar analogs were used as the divisor in the reduction to "relative flux" of all the spectra taken at the Galileo telescope in Asiago. The figures in the volume depict spectra resulting from the division: (comet flux / Solar Analog flux).\\

\section{IMAGING}
This volume is accompanied by numerous images, with at least a couple provided for each comet, along with their respective explanatory captions. The sensors used on the telescopes for imaging were all monochromatic, which means they produced grayscale images. The color figures presented in the volume are the result of the creation of tricolor images composed of individual shots taken through photometric bandpass filters following the Johnson-Cousins ($B, V, R, I$) or Sloan ($u, g, r, i, z$) standards. Other images included in the volume were also captured using standard photometric filters (Fig. 4, 5, 6, 7). The imaging sessions took place during observational nights using the instruments at Cima Ekar, situated a few kilometers southeast of Asiago, at an altitude of 1366 meters, with the IAU-MPC code 098. The Copernico telescope with a diameter of 182 cm and its Asiago Faint Objects Spectrograph and Camera (AFOSC) instrument was employed for imaging. It features an Andor iKon-L936 BEX2-DD-9HF camera equipped with a back-illuminated E2V CCD42-40 sensor, providing 2048×2048 pixels with a 13.5 $\mu m$ side and a resolution on the celestial plane of 0.25$"$/pixel.\\
The Schmidt telescope with diameters of 67/92 cm was equipped with a Moravian CCD camera featuring a KAF-16803 sensor. This sensor offers 4096×4096 pixels with a 9x9 $\mu m$ size, resulting in a resolution of 0.87$"$/pixel on the celestial plane.\\
It should be noted that some images were captured using other telescopes in the 50-cm class, and the specific location is indicated in the image captions. All original images underwent calibration using master bias and dark frames, and flat field corrections.\\
For all imaging sessions, differential tracking was employed, adjusted to the comet's speed relative to the stars. If several images of a comet were taken with the same filter in the same observation session, they were co-added after re-centering them on the cometary nucleus. This procedure allows to significantly increase the signal-to-background ratio. During post-processing, an additional realignment of the images was performed on the optocenter of the comet nucleus, ensuring a final result with sub-pixel precision. These processed images reveal stars as streaks, making it easy to discern the direction of the comet's motion. The table below lists the specifications of the photometric filters used:

\begin{table}[h!]
    \centering
    \begin{tabular}{|c c c c|}
    \hline
    \textbf{Filter} & \textbf{CWL} & \textbf{FWHM} & \textbf{Remarks}\\
     & [nm] & [nm] & \\
     \hline
     \hline
     u' & 354.3 & 320-385 & Sloan \\
     B & 436.1 & 89 & Bessel \\
     V & 544.8 & 84 & Bessel \\
     g' & 477.0 & 401-550 & Sloan \\
     r' & 623.1 & 555-695 & Sloan \\
     i' & 762.5 & 690-820 & Sloan \\
     z' & 913.4 & > 820 & Sloan \\
     \hline
    \end{tabular}
    \caption{Filters used on both the Copernico and Schmidt telescopes at Cima Ekar (Asiago). The CWL (Central Wavelength) column specifies the central wavelength of the filter's passband.}
    \label{tab:filters}
\end{table}
% TABELLA FILTRI MANZINIANI UUUUUU <----
\noindent The procedure is slightly different for some images taken with other telescopes in the 50 cm class; the location is indicated in the caption of the relevant images.\\
Several images accompanying the volume result from the application of a simple photometrically calibrated trichromy in the R channel (Sloan r' filter), G channel (Johnson Vj), and B channel (Johnson Bj). These images provide a sufficiently realistic representation of how the comet would appear in the sky if one had a calibrated eye sensitive to low light conditions.\\
Other figures result from processing with the Larson-Sekanina mathematical algorithm, which is one of the most commonly used filters for the morphological study of comets' coma (Larson S. \& Sekanina Z., AJ, 1984). The application of this filter highlights micro variations in the brightness within a comet's coma, enabling a detailed study of morphological structures within the inner coma, near the nucleus.\\
In images processed with this algorithm, star trails (which already appear as bright/white in the original shots) are accompanied by two symmetrically positioned dark/black trails on either side, which are due to the equation applied by the filter (Fig. 8, Fig. 9).\\
These image processing techniques reveal morphology of the inner coma in nearly every comet, which can be traced back to its source on the comet nucleus. They are a useful method for studies aimed at identifying axes of symmetry correlated with the rotation of the nucleus and the orientation of its axis.\\
The volume also contains some figures resulting from isophote visualization, which highlights the extent of the nebulosity (coma+tail) around the comet nucleus along with asymmetries resulting from dust and gas emissions from active areas on the nucleus. The isophote traces have a discrete and precise step in ADU (Analog-to-Digital Units), repeated throughout the image. The visualization of the first isophote corresponds to a brightness just a few ADU above the sky background (Fig. 10, 11).
\newpage

\section{REPRESENTATION OF IMAGES}
\subsection{TRICHROME IMAGES}

\begin{SCfigure}[0.8][h!]
    \centering
    \includegraphics[scale=0.138]{img_intro/fig_4_E3_20230211_BVr_DDP.jpg}
    \caption{Fig.4 A trichrome image of comet C/2022 E3 (ZTF). The three monochromatic images composing it are derived from shots using Bj, Vj, and r’ photometric filters at the Schmidt 67/92 telescope at the Cima Ekar Observatory (Asiago). Individual frames with exposure times of 60 and 120 seconds were all aligned using the optocenter of the comet as the reference point, which is the brightest photometric point presumed to be the nucleus.}
    \label{BAH}
\end{SCfigure}
% Fig. 4.  
\noindent A trichrome image immediately highlights the different typical regions of a comet: the nucleus, the coma, and the tail. The tail appears reddish due to the presence of micrometer-sized dust particles that scatter and reflect sunlight. The greenish-blue of the coma, on the other hand, results from the fluorescence of biatomic carbon (C$_2$) molecules, which are found in large quantities there.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.083]{img_intro/fig_5-E3_20230211_BVr_B_DDP.jpg}
    \includegraphics[scale=0.083]{img_intro/fig_6_E3_20230211_BVr_R.jpg} 
    \includegraphics[scale=0.083]{img_intro/fig_7_E3_20230211_BVr_V.jpg}
    \caption{Fig.5,6,7}
    \label{BAH}
\end{figure}

%Fig. 5, Fig. 6, Fig. 7  
\noindent The trichrome image above is derived from the merging in the RGB channels of the monochromatic shots shown here, respectively taken with Bj, Vj, and r’ filters. Each of them highlights specific details and features that are only visible in the specific spectral bands used. North is at the top, and east is to the left.


\subsection{THE LARSON-SEKANINA ALGORITHM}
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.55]{img_intro/fig_9-67p_20220127_(u+B)Vr.jpg} 
    \includegraphics[scale=0.55]{img_intro/fig_8-67p_20220127_(u+B)Vr_ls20.jpg}
    \caption{Fig.8,9}
    \label{BAH}
\end{figure}
%Fig. 8, Fig. 9
\noindent These two figures provide a very clear illustration of what is "hidden" within a comet's coma.\\
On the left is a trichrome image of comet 67P (Churyumov-Gerasimenko) taken on January 27, 2022 (Copernico telescope, Cima Ekar - Asiago). The application of the Larson-Sekanina algorithm at an angle of 20° highlights some morphological structures within the inner coma. These structures directly originate from highly active regions located on the nucleus, emitting large quantities of gas and dust. The dust particles maintain their spin and velocity until the pressure from solar radiation pushes them back, forming the comet's tail.\\
In images processed with this algorithm, the star trails, which appear bright in the original shots, are accompanied on both sides by two symmetrical dark trails due to the equation applied by the filter. In this specific case, with the comet in a rich star field, the dark trails have been partially removed to better reveal the morphological structures. North is at the top, and east is to the left.\\
\clearpage
\subsection{ISOPHOTE VISUALIZATION}
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.8]{img_intro/fig_10-20191023_Copernico_clear_2x.jpg} 
    \includegraphics[scale=0.8]{img_intro/fig_11-20191023_Copernico_clear_iso500_2x.jpg}
    \caption{Fig.10,11}
    \label{BAH}
\end{figure}

%Fig. 10, Fig. 11  
\noindent The same image is represented in two different ways.\\
Left: The original image, which is a sum of individual frames of comet 260P, has had a DDP (Digital Development Process) filter applied to it. This filter gives the images an appearance similar to those on film. It is useful for identifying low-contrast details within a comet's coma.\\
Right: The isophote visualization involves setting the lower-level isophote to a value just a few ADUs (Analog-to-Digital Units) higher than the sky background. This highlights the actual extent of the comet's coma along with asymmetries in the distribution of brightness related to emissions of gas and dust from the nucleus. The number of pixels between the minimum and maximum values within which the isophotes are developed allows for photometry of these diffuse objects.\\
The isophotal lines are spaced with a constant step across the entire image. In Fig. 11, they are spaced 500 ADUs apart and are represented in false color, with blue indicating the minimum brightness values in the image.\\
This image is a composite of shots taken at the Asiago Astrophysical Observatory (MPC-098, Italy) with the 1.82-m Copernico telescope.\\
North is at the top, and east is to the left.\\
\clearpage 
\section{COMET DATA SHEETS}
In spectral data for 37 comets observed with the Galileo telescope at the Asiago Astrophysical Observatory are presented. In total, there are 133 spectra obtained over ten years of observations.\\
For easier reference, the pages dedicated to each comet follow an identical structure.
The first page features two tables, with the first one listing the orbital elements of the comet obtained from the JPL Horizon website (e.g., \url{https://ssd.jpl.nasa.gov/tools/sbdb_lookup.html#/?sstr=260p}). \\
The second table provides position and distance ephemerides for two key dates in the transit of the comet: perihelion and perigee. It also includes values for the elongation of the comet from the Sun, the phase effect on the nucleus, and the Earth's position relative to the comet's orbital plane. These data allow for the visualization of the comet's position in the sky.\\
The first page also includes a diagram of the comet's orbit, which size can be directly compared to the orbits of Earth and Jupiter (credits: NASA/JPL-Caltech). The orbit and positions of these three celestial bodies are indicated for the date of the comet's perihelion (\url{https://ssd.jpl.nasa.gov/tools/orbit_viewer.html}). In a couple of cases, the scale has been enlarged to include the orbits of Saturn and Uranus.
Vertical lines are added alongside the comet's orbit to reference its position on the $z$-axis (the short side of the image) and in relation to the plane of the ecliptic. The figure provides information on when the comet is "above" or "below" the Earth's ecliptic.\\
A couple of images of the comet are shown on the second page of each data sheet. Each figure includes the exact orientation and a scale in kilometers measured on the plane of the sky at the comet's distance at the time of imaging. For a more precise description of the visualization methodologies, you can refer to the previous sections.\\


\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{12}{|c|}{Observation details}                      \\ \hline 
\hline
$\#$  & date          & r     & $\Delta$ & RA     & DEC     & elong & phase & PLang& config  &  PA & exp \\
      & (yyyy-mm-dd)  &  (AU) & (AU)     & (h)    & (°)     & (°)   & (°)   &  (°)   &       &  (°)  & (s)\\ \hline 

1 & 2023-07-23 & 3.850 & 3.539 & 18.22 & +55.79 & 100.15 & 15.06 & -11.04 & A & 167.50 & 600\\
2 & 2023-08-11 & 3.652 & 3.404 & 17.75 & +54.77 & 96.03 & 16.03 & $-$14.64 & A & 93.36 & 900 \\

\hline
\end{tabular}
\caption{Fig.12}
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{|c c c c c|}
        \hline
        \textbf{Lines/mm} & \textbf{Blaze wavelength} & \textbf{Dispersion} & \textbf{Spectral Range} & \textbf{Identification}\\
         & [\AA] & [\AA/px] & [\AA] & \\
        \hline
        \hline
        300 & 5000 & 2.25 & 3500-7000 & A \\
        600 & 4500 & 1.15 & 4250-6590 & B \\
        1200R & 6825 & 0.6 & 5750-7000 & C \\
        1200B & 4000 & 0.6 & 3820-5020 & D \\
        \hline   
    \end{tabular}
    \caption{Fig.13}
    \label{tab:identification}
\end{table}

\noindent On the following pages, for each comet we include a table containing details of all the observations conducted with the spectrograph of the Galileo telescope. Here, you can find the date, the comet's distance from the Sun and Earth, the equatorial coordinates, and the elongation in degrees from the Sun at the time of each observation. In the eighth and ninth columns, the phase angle on the comet's nucleus and the angle from which the comet is observed from Earth relative to the comet's orbital plane are reported. Positive values indicate that the observer is located above the object's orbital plane (see example in Fig. 12).\\
Three columns have been added to the table on the third page to indicate the configuration of the spectrograph and the data of the capture. These columns respectively show the grating used for the observation, the slit angle (E-W = 0°, N-S = 90°), and the exposure time for each spectrum.\\
The setup of the Galileo telescope's B\&C spectrograph can be varied to suit the observer's needs, and an identification letter (A, B, C, D) has been associated with each configuration. The same letter is also indicated in the table on the third page of each comet's data sheet (see example in Fig. 13).\\
A representative spectrum of each comet is graphically presented on the last page of the section. The major emission lines due to molecules and atoms present around the nucleus and in the inner coma of the comet can be easily identified. The spectra are presented with relative flux on the ordinate axis (comet flux divided by Solar Analog flux) and wavelength on the abscissa axis. If the flux is too intense, as is typically the case for the CN $\lambda$3880 line, the $y$-axis has been truncated to better visualize even the weaker emission lines.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.55]{img_intro/fig_14-spettro_20181128_46P_300tr.png} 
    \includegraphics[scale=0.57]{img_intro/fig_15-bande_e_continuo_c2014q2_Lovejoy.png}
    \caption{Fig.14,15}
    \label{BAH}
\end{figure}

%Fig. 14, Fig. 15
\noindent In Figure 14, a typical spectrum of comet 46P (Wirtanen) taken on November 28, 2018, in configuration A (Figure 13) with a diffraction grating of 300 lines/mm is visible. To facilitate comparison and identification, Figure 15 provides indications of the relevant regions of the major molecular bands observable in a comet spectrum. It also indicates three areas of the spectrum where conventionally the continuum can be "read": the Blue Continuum between 4300 and 4510 Å, the Green Continuum between 5200 and 5320 Å, and the Red Continuum between 7060 and 7180 Å. On the ordinate axis, the values represent the flux density identified as the value in $erg \ cm^{-2} \ s^{-1} \ $\AA$^{-1}$.
\clearpage
\section{SPECTRA AT THE GALILEO TELESCOPE}
For a more in-depth study of celestial objects, the setup of the B\&C spectrograph at the Galileo telescope can be substantially modified to suit the observer's needs. In the case of comet observations, it is particularly interesting to have the possibility of studying them with gratings of different resolutions to investigate the fine structure of lines in their spectra (Figure 13).\\
At the same time, as in the case of this volume, collecting spectral analyses of many comets allows to observe significant variations in the species and quantity of molecules emitted, depending on the internal physical structure of the comet nucleus and its distance from the Sun.\\
To provide an example of the possibilities offered by the Galileo telescope's instrumentation, below are some spectra of bright comets (thus with good S/N) taken with different gratings and in different parts of the spectrum.\\
Some graphical sections of spectra centered at 3880 Å around the main emission line due to CN, at 6300 Å for the oxygen [O I] line emission, and at 5890 Å for the presence of the sodium (Na) line doublet, allow for detailed analysis and comparison of the regions around these lines.
Using the method established by Haser, a $Q$ value can be calculated for each molecule under examination, which represents the emission of dust and gas measured in kg/sec (Combi, Comets II, 2005). However, this analysis goes beyond the immediate goals of this volume. The authors' intention is to make dozens of comet spectra available to the scientific community, which can be requested at any time for specific research purposes.\\
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.32]{img_intro/fig_16_E3_20221019_Galileo_300tr_scala_min.png} \\
    \includegraphics[scale=0.32]{img_intro/fig_17_E3_20230129_Galileo_1200B_scala_minima.png}\\
    \includegraphics[scale=0.40]{img_intro/fig_18_c2020t2_20210731_Galileo_300tr_CN.png} 
    \includegraphics[scale=0.40]{img_intro/fig_19_E3_20230129_Galileo_1200B_CN.png}
    \caption{Fig.16,17,18,19}
    \label{BAH}
\end{figure}

%Fig. 16,17,18,19 
\noindent Fig. 16, Fig. 17, Fig. 18, Fig. 19 Comparison of different spectrograph setups applied to the Galileo telescope. Respectively:\\
Comet C/2022 E3, spectrum from October 19, 2022, 300 lines/mm grating, dispersion 2.25 \AA/pixel. \\
Comet C/2022 E3, spectrum from January 29, 2023, 1200 lines/mm grating, dispersion 0.6 \AA/pixel, Blue region of the spectrum.\\
Comet C/2020 T2, spectrum from July 31, 2021, CN line, 300 lines/mm grating, dispersion 2.25 \AA/pixel.\\
Comet C/2022 E3, spectrum from January 29, 2023, CN line, 1200 lines/mm grating, dispersion 0.6 \AA/pixel.\\
All spectra result from the division of the recorded comet flux by that of the star defined as Solar Analogue; the scale on the ordinate axis is therefore a relative value.\\
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.32]{img_intro/fig_21_e3_20230228_Galileo_1200R.png} \\
    \includegraphics[scale=0.32]{img_intro/fig_21_e3_20230228_Galileo_1200R.png}\\
    \includegraphics[scale=0.40]{img_intro/fig_22_19P_20220222_Galileo_300tr_OI.png} 
    \includegraphics[scale=0.40]{img_intro/fig_23_e3_20230228_Galileo_1200R_OI.png}
    \caption{Fig.20,21,22,23}
    \label{BAH}
\end{figure}

%Fig.  20,21,22,23 
\noindent Fig. 20, Fig. 21, Fig. 22, Fig. 23
Comparison of different spectrograph setups applied to the Galileo telescope. Respectively:
Comet 19P, spectrum from February 22, 2022, 300 lines/mm grating, dispersion 2.25 \AA/pixel.\\
Comet C/2022 E3, spectrum from February 28, 2023, 1200 lines/mm grating, dispersion 0.6 \AA/pixel, Red region of the spectrum.\\
Comet 19P, spectrum from February 22, 2022, O I lines, 300 lines/mm grating, dispersion 2.25 \AA/pixel; in addition to the O I lines (6300 Å+6364 \AA), there is also the emission from NH at 6327 \AA. \\
Comet C/2020 E3, spectrum from February 28, 2023, O I lines, 1200 lines/mm grating, dispersion 0.6 \AA/pixel.\\
All spectra result from the division of the recorded comet flux by that of the star defined as Solar Analogue; the scale on the ordinate axis is therefore a relative value.\\
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.40]{img_intro/fig_24_e3_20230107_Galileo_1200R_Na_200micron.png} 
    \includegraphics[scale=0.40]{img_intro/fig_25_e3_20230107_Galileo_1200R_Na_400micron.png}\\
    \includegraphics[scale=0.40]{img_intro/fig_26_e3_20230107_Galileo_1200R_Na_600micron.png} 
    \includegraphics[scale=0.40]{img_intro/fig_27_e3_20230107_Galileo_1200R_Na_800micron.png}
    \caption{Fig.24,25,26,27}
    \label{BAH}
\end{figure}
%Fig.  24,25,26,27,28 
\noindent Emissions due to the Sodium doublet (D1 at 5986 \AA\,and D2 at 5980 \AA) are rarely observed and usually in comets approaching the Sun at a distance greater than 1 AU. In this case, the presence of sodium emissions on comet C/2022 E3 at 1.115 AU from the Sun on January 7, 2023, was highlighted with the Galileo telescope.\\
The spectrograph setup allows for varying the slit width, as shown in the images from top left: 200$\mu$, 400$\mu$, 600$\mu$, 800$\mu$. Increasing the slit width corresponds to analyzing a larger area of the coma around the nucleus.\\
The lower figure provides a direct comparison of the results with different slit widths. The ordinate scale is the same for the first 4 figures.
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.40]{img_intro/fig_29_m3_20201112_Galileo_300tr_Na.png} 
    \includegraphics[scale=0.40]{img_intro/fig_30_m3_20201117_Galileo_1200R_Na.png}\\
    \includegraphics[scale=0.40]{img_intro/fig_31_v2_20230102_Galileo_1200R_Na.png} 
    \includegraphics[scale=0.40]{img_intro/fig_32_t2_20200104_Galileo_300tr_Na.png}
    \caption{Fig.29,30,31,32}
    \label{BAH}
\end{figure}
%Fig. 29,30,31,32 
From top left: C/2020 M3 on November 12, 2020, at 1.296 AU from the Sun (300 lines/mm grating), C/2020 M3 on November 17, 2020, at 1.313 AU (1200 lines/mm grating R), C/2020 V2 on January 2, 2023, at 2.646 AU (1200 lines/mm grating R), C/2017 T2 on October 4, 2020, at 2.667 AU (300 lines/mm grating).
The ordinate scale is different for each figure.

\newpage











                                  
